VELTAIR: Towards High-Performance Multi-tenant Deep Learning Services via Adaptive Compilation and Scheduling

Deep learning (DL) models have achieved great success in many application domains. As such, many industrial companies such as Google and Facebook have acknowledged the importance of multi-tenant DL services. Although the multi-tenant service has been studied in conventional workloads, it is not been deeply studied on deep learning service, especially on general-purpose hardware. In this work, we systematically analyze the opportunities and challenges of providing multi-tenant deep learning services on the general-purpose CPU architecture from the aspects of scheduling granularity and code generation. We propose an adaptive granularity scheduling scheme to both guarantee resource usage efficiency and reduce the scheduling conflict rate. We also propose an adaptive compilation strategy, by which we can dynamically and intelligently pick a program with proper exclusive and shared resource usage to reduce overall interference-induced performance loss. Compared to the existing works, our design can serve more requests under the same QoS target in various scenarios (e.g., +71%, +62%, +45% for light, medium, and heavy workloads, respectively), and reduce the averaged query latency by 50%.

==> Acknowledgements.tex <==
%\section{Acknowledgements}


==> CharacterizingInterference.tex <==
\section{Co-locating Interference Characterizing}
To resolve the performance downgrade caused by interference, we first need a method to evaluate how serious the interference is that the system is currently suffering. 
In this section, we'll first illustrate the significance of the interference existing in op co-locating, then we will analyze the root cause of this kind of interference. Finally, we will give a simple interference model used in this paper.
\subsection{Significance of Interference}
Use heatmap and end-to-end QoS.
\subsection{Interference Factors Analysis}
Analyze based on performance counter, mainly we should draw to this conclusion: \textbf{Using L3 Bandwidth and CPU Util can determine the interference behavior of an op} and \textbf{There exists linear relation when scaling 1 background op to multiple background ops.}.
\subsection{Interference Model}
We use a simple linear model to characterize the model, and get relatively high accuracy in determining which op suffered the most and to what extend they suffered.

==> Methodology.tex <==
\section{Enabling Low-Interference Multi-Tenant Service Co-Locating}
This section mainly describes our design and corresponding insight to serve multiple deep learning task with low interference. First, we will analyze the optimization space.
% \subsection{Optimization Space Exploration and Problem Formalization}
% First, we will discuss the optimization space that necessary for improving the performance in this work and try to formalize our problem with mathematics notation for further optimization. 
% \subsubsection{Version Switching Under Interference}
% Currently, the concept of switching implementation versions to handle interference is absent in deep learning service providing and corresponding compiler and runtime scheduler. At compiling stage, most state-of-the-art compilers try to find an operator implementation (code transformation and instruction schedule) that maximizes the overall float point performance, including Tiramisu auto-scheduler, TVM auto-scheduler, TensorComprehensions, etc. After the best-performance implementation is found, the runtime scheduler will fix the implementation version to use, and only care about the exclusive and shared resource allocation. However, as we've observed, some of the operators suffer from severe interference when they are co-located with other operators, making this methodology has sub-optimal optimization under multi-tenant serving scenarios. 
% On the other hand, according to our observation, multiple implementations of the same operator behave differently to interference. Some implementations have lower performance when they execute alone but have only a slight performance drop when they suffer from heavy interference pressure as illustrated in figure~\ref{fig-MultiVersionNecessity} (b), and we define these operators (Version 5 in the figure) to be \textbf{Interference Tolerant}. In this work, we try to explore the possibility of finding operator implementations with different \textbf{Interference Tolerance} and dynamically selecting the version of implementation with different interference tolerance according to system profile, SLA satisfactory rate, etc. 

% So, we first launch the standard TVM auto scheduler procedure multiple times for verification with 2048 iteration every time (to make sure the auto scheduler can return "good enough" implementations). After we've found multiple implementation versions for convolution and matrix multiplication operators appear in the networks we used in the evaluation, we then profiled the behavior of these implementation versions in different interference pressure levels by launching different background operators as interference. In figure~\ref{fig-MultiVersionAndStackedBar}, we demonstrated the behavior of 7 convolution operators with 8 different implementation versions respectively facing different interference pressure. 8 curves (representing 8 implementation versions) form the best choice for the operator facing different interference pressure. We also can use fewer implementation versions to reach 90\% of the best performance (The titles of every sub graphs show the necessary number of versions to reach 90\% of the performance). 
% The last sub-graph of the figure~\ref{fig-MultiVersionAndStackedBar} illustrated the required version number to satisfy different performance losses. If we only use one version for every operator, we are likely to lose 70\% performance in various interference pressure.
% \begin{figure*}[h]
%     \centering
%     \includegraphics[width=0.24\linewidth]{VerNum=1,OPID=12-eps-converted-to.pdf}
%     \includegraphics[width=0.24\linewidth]{VerNum=2,OPID=16-eps-converted-to.pdf}
%     \includegraphics[width=0.24\linewidth]{VerNum=2,OPID=48-eps-converted-to.pdf}
%     \includegraphics[width=0.24\linewidth]{VerNum=3,OPID=13-eps-converted-to.pdf}\\
%     \includegraphics[width=0.24\linewidth]{VerNum=3,OPID=37-eps-converted-to.pdf}
%     \includegraphics[width=0.24\linewidth]{VerNum=3,OPID=43-eps-converted-to.pdf}
%     \includegraphics[width=0.24\linewidth]{VerNum=4,OPID=30-eps-converted-to.pdf}
%     \includegraphics[width=0.24\linewidth]{LossAndVersionNum-eps-converted-to.pdf}
%     \caption{\label{fig-MultiVersionAndStackedBar} Sub figure 1 to sub figure 7 demonstrate 7 different operators' behavior with interference, each operator has 8 different implementations. We define the best performance of an operator by choosing the highest TFLOPS under every interference level, and the shadow area represents the 90\% to 100\% performance. To find out how many versions an operator needs at least to reach 90\% of the best performance, we examine the minimal number of the line that can fully cover the 90\% performance area. For example, for convolution operator $ C_{in}=512, C_{out}=512, H_{in}\times W_{in}=14\times 14, Kernel=(3\times 3) $ (the $ 4^{th} $ sub figure), if we use only version 3 and version 4, we can not reach 90\% of the best performance once the interference level exceed 40. The last sub figure illustrate the necessary version number distribution of 170 different convolutions appear in the networks we use in evaluation under different performance downgrade accept rate. If we use only 1 version as most of the existing work do, we are likely to lose over 70\% performance. \FIXME{Remove subfig 1 to subfig 7, add boxplot of version's perf loss against the best, can use 2 subfigs as example}}
% \end{figure*}
% \subsubsection{Resource Allocation Preference}
% In the scenarios of providing online service, existing works have proposed various CPU core allocation strategies corresponding to their optimization objectives and hardware multiplexing manners. For example, some works use temporal multiplexing and maximize the CPU core usage so that the task monopolizing the hardware can finish ASAP. Others use spatial multiplexing and limit the CPU core usage to an exact number that SLA requirements are satisfied to allow more tasks to share the hardware resources. Preemption is also often considered for a lower response latency, at the cost of increasing system overhead. 


% \subsubsection{Scheduling Grain}
% To launch and schedule tasks onto the hardware, we have several choices on which grain should we schedule the tasks. To schedule the task at a task grain, we handle a task as an atomic unit, allocating identical resource to all components in the task and ignoring the detailed structure inside the task makes it not only simpler to allocate resources but also faster to make schedule decisions, thus reduce the overhead. However, scheduling the task at coarse grain means we should wait for some task to complete to release necessary resources which leads to high response latency (or we should let the tasks with higher priority preempt the hardware by use all CPU resource in temporal multiplexing or limit others' resource in spatial multiplexing, which introduce significant overhead), following reasons make it even more in-appropriate to the scenario of online deep learning service providing for following reason.
% \begin{itemize}
%     \item Deep learning tasks consist of inference of deep neural network which is more time costing comparing to traditional interactive tasks, making the problem of response latency even more severe. 
%     \item Deep neural networks are formed from multiple layer of computation nodes with different computation characteristics, which should be considered in resource allocating and operator scheduling for a better performance.
% \end{itemize}
% By scheduling the tasks at layer or even sub-layer grain the system can respond to new tasks with much lower latency, moreover, the system can have more optimization opportunities including operators reordering and resource re-arranging, etc., of course, at the cost of searching in a much larger space which leads to higher runtime scheduling overhead. 
% Moreover, according to our observation, different layers in tasks have significant difference in CPU core requirement to satisfy QoS requirement as illustrated in figure~\ref{fig-CoreNumUseAndUtil} (a) (We calculate each layer's QoS according to its float point operation count compare to the whole network), and this fluctuate CPU core usage results in severe resource allocation conflict which the available slot of the hardware is less than the operators' CPU core requirement to meet their QoS target. In that case, we either launch the operator anyway with sub optimal performance or preempt the resource from those tasks likely to complete in advanced. However, both method will bring significant overhead including context switching when preempting resource from on-going tasks, threads competition when launching threads to less hardware cores, etc. To solve this problem, we propose the scheduling strategy sub-model by sub-model, the formation of sub-model will be detailed in following chapters. By forming layers into sub-model, the QoS requirement of layers in sub-model can be relaxed, making the overall CPU core requirement more smooth, thus reducing the resource allocation conflict, as illustrated in figure~\ref{fig-CoreNumUseAndUtil} (a). 
% Figure~\ref{fig-CoreNumUseAndUtil} (b) is CPU utilization and efficiency of an experiment of launching 300 tasks in the same period with the same time interval. Obviously, the CPU utilization of layer-by-layer scheduling is almost 100\%, but the efficiency is less than half. However, for sub-model based scheduling, the CPU can be used with much more efficiency, moreover, the utilization is lower which means we can co-locate even more tasks onto the CPU. Finally, the overall completing time of sub-model based scheduling is shorter by over 50\% than layer-by-layer scheduling.
% However, according to our observation of a simple verification experiment in which we implement a layer grain scheduling algorithm with sub-layer (tile) grain preemption enabled proposed in Planaria~\cite{Planaria}, scheduling at layer grain achieves sub optimal performance. According to figure~\ref{fig-StrategyCmpAndUsage}
%  (a), comparing to a simple sub-model grain scheduling algorithm, the average and tail latency of layer grain scheduling algorithm increase by $ 15\%-20\% $ ($ Avg.:~18.74~ms \rightarrow 22.04~ms, \Delta_{Avg.~Latency}=3.3~ms$), since the CPU core are exactly allocated to satisfy the QoS target, the gap in latency influence the QoS satisfaction rate at different QPS dramatically. 
%  The reason of sub optimal performance of layer grain scheduling algorithm is increasing CPU resource preemption compared to sub-model grain scheduling. According to figure~\ref{fig-StrategyCmpAndUsage} (b), the CPU core requirement of layer grain scheduling is much more fluctuating than sub-model grain scheduling, which is more likely to trigger resource allocation conflict and use preemption to resolve. The conflict rate is about $ 25\% $ in layer grain scheduling illustrated in figure~\ref{fig-StrategyCmpAndUsage} (a), representing almost one-fourth of the operator encounter resource conflict. However, sub-model grain scheduling can avoid such conflict. 
%  To verify our assumption, we profile 104 operators' performance of normal execution and switching CPU core resource when executing, figure~\ref{fig-OverheadAndUtil} (a) shows that switching CPU core resource have 220 us average overhead. Combining $ 25\% $ conflict rate and 220 us conflict overhead, we use ResNet-50 (55 operators) as exemplification. $ \Delta_{Avg.~Latency~Estimated}=55\times 25\%\times220=3.03~ms $, which matches the measure $ 3.3~ms $ well. We also measure the CPU utilization snapshot when evaluating. We launch 30,000 tasks in total with no arriving interval and measure completing time. According to figure~\ref{fig-OverheadAndUtil} (b), layer grain scheduling have $ 12.5\% $ efficiency (user space CPU utilization) drop comparing to sub-model grain scheduling, since the efficient computation of two strategies should be similar and they actually are (the area covered by two curves is similar), the completing time of layer grain scheduling is $ 24.2\% $ longer. 
% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.49\linewidth]{TwoStrategyCmp-eps-converted-to.pdf}
%     \includegraphics[width=0.49\linewidth]{CPUCoreUsage-eps-converted-to.pdf}
%     % CoreNumPlot/plot.py & plot2strategyres.py
% 	\caption{\label{fig-StrategyCmpAndUsage} (a) QoS satisfaction rate and latency of different scheduling grain (we implement a layer-by-layer strategy according to Planaria~\cite{Planaria}), scheduling by sub model can increase the QPS with $ >95\% $ by 2$\times$. (b) CPU core usage to satisfy QoS target of ResNet-50 and GoogLeNet, scheduling at sub-model grain has much more smooth core usage pattern than scheduling at layer grain. }
% \end{figure}
% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.49\linewidth]{Overhead-eps-converted-to.pdf}
%     \includegraphics[width=0.49\linewidth]{CPUUtilEffi-eps-converted-to.pdf}
%     % CoreNumPlot/plot.py & plot2strategyres.py
% 	\caption{\label{fig-OverheadAndUtil} (a) Measured overhead of switching CPU core resources when an operator is running, which is mainly caused by new threads forking and launching. (b) Total CPU utilization and user space CPU utilization of two scheduling grain, the effective computation (area covered by two curve) is similar, but the efficiency of scheduling at layer grain is lower than scheduling at sub model grain by $ 20\% $.}
% \end{figure}
% \subsubsection{Problem Formalization and Notations}
% In this part, we will give the problem a formal definition, first, we will describe the scenario we handle in mathematics symbol.
% Given a time period $ T $, the task $ t $ with QoS set to $ qos_{t} $ will arrive following Poisson Distribution, and the $ \lambda $ of Poisson distribution is set to the Query Per Second (QPS) of the system, and in total $ S $ tasks arrived in this time period. Under this circumstance, we examine the ratio of tasks' QoS requirements that have been satisfied $ r $ under a $ \lambda $ configuration. The task $ t $'s QoS $ qos_{t} $ is satisfied means the actual execution time of t $ time_{t} $ and $ qos_{t} $ satisfy the relation of $ time_{t} \leq qos_{t} $. Since one task consist of several layers, we can also calculate layers' QoS $ qos_{t}\lbrack i \rbrack, i\in\lbrack 1, t.length \rbrack $ according to layers' float point operation count $ fp\_count_{t}\lbrack i \rbrack, i\in\lbrack 1, t.length \rbrack $ by $ qos_{t}\lbrack i \rbrack=qos_{t} \times \frac{fp\_count_{t}\lbrack i \rbrack}{\sum_{j\in\lbrack 1, t.length \rbrack}(fp\_count_{t}\lbrack j \rbrack)} $.
% Given a system with $ C $ CPU cores in total and $ c $ cores as minimum unit to allocate, we allow at most $ P=\frac{C}{c} $ tasks running in parallel, for convenience, we use $ t\_running_{ts}[0:P-1] $ to represent the running tasks of the system at a timestamp $ ts $. For switching version, we prepare at most $ V $ different implementation version for an operator. 

% In table~\ref{tab-Strategies}, we conclude and list some existing work and their scheduling/optimization options following our optimization framework. The meaning of notation is:
% \begin{itemize}
%     \item Multiplexing Manners (MM): Indicate whether the strategy applies Temporal Multiplexing or Spatial Multiplexing. Since the optimization objective of CPU core is closely related to multiplexing manners, we list them in the same column.
%     \item Preemption (PR): Indicate whether the strategy allow new task to preempt the resource of on-going tasks.
%     \item Scheduling Grain (GR): Indicate the scheduling grain of the strategy, we categorize existing works' option into 4 group: Model (M), Sub-Model (SM), Layer (L), Sub-Layer (SL).
%     \item Version Switching (VER): Indicate whether the strategy consider using multi-version operators implementation to relax interference problem. 
% \end{itemize}

% \begin{table}[h]
% 	\caption{\label{tab-Strategies} Various strategies and their optimization options.}
% 	\begin{center}
% 	\begin{tabular}{|c|c|c|c|c|}
% 	    \hline
	    
% 		\hline
%         MM & PR  & GR & Ver. & Strategy\\
%         \hline
%         T-$ max $ & Yes & M & No & PREMA \\
%         T-$ max $ & No & SL & No & AI-MT* \\
%         S-$ min $ & Yes & SL** & No & Planaria* \\
%         S-$ min $ & No & M/L*** & Yes & Protean \\
%         S-$ min $ & No & M/L*** & No & Parties \\
%         S-$ min $ & Yes & SM & Yes & \proj{}\\
%         \hline
%     \end{tabular}\\
%     \end{center}
%     \emph{* These 2 are software-hardware co-design works, and they evaluate their design on their own-designed systolic architecture.\\
%     ** Planaria schedule the model on layer grain, but it allow the layer to preempt the hardware at tile grain when the estimated resource can not fit the available slot on the hardware, so we mark it as Sub Layer (SL).\\
%     *** Protean and Parties mainly handle traditional interactive application scenarios, in deep learning service, we can either define a layer as a task or a whole as a task.\\}
% \end{table}

\subsection{\proj{} Compiling and Scheduling Strategy}
\PBox {
    \textbf{Core Insight A}: Interference of co-locating multiple deep learning task can be relaxed by switching implementation version of operators.
}
\subsubsection{Finding Candidate Version at Compiling Stage}
To get the heuristic to find implementation versions to handle different interference levels, we first find multiple implementation versions of operators with no extra heuristic to examine the relationship between their behavior to interference and their compiler flags. In this work, we mainly use TVM Auto Scheduler~\cite{Ansor} to find the code transformation and scheduling automatically. According to Halide~\cite{Halide}, there is a trade-off between parallelism, locality, and computation efficiency when generating code. Since we do not consider fusing multiple reduction layer together, no redundant computation need to be considered. So, we mainly focus on \textbf{unroll/parallel pragma} and \textbf{blocking/tiling size} of the implementation representing parallelism and locality respectively of an implementation.
We launched several operators in 2 situations: no interference and heavy interference (by launching a "background" operator to give interference pressure) and find the best-performed implementation of these operators by profiling. According to figure~\ref{fig-MultiVersionFinding} (a), most of the operators will choose the implementation with a larger tiling size and lower parallelism to handle heavy interference, and it should be noted that the closer an implementation is to the upper right in the figure, the better this implementation is, since it can use less shared resources and leverage more parallelism. That's because given larger blocks, the total number of blocks will decrease, resulting in decreased LLC access thus relaxing bandwidth occupation. 
Though the LLC capacity requirement will increase, according to figure~\ref{fig-L3Prof} (a), we use Intel CAT to limit the L3 cache line available to an application and find that the performance will only drop when we allow the application to use only one cache line (This experiment is done on a Xeon $ 2^{nd} $ Scalable Processor since Threadripper CPU does not support cache line adjustment). What's more, the Threadripper CPU we use have a huge amount of L3 Cache of $ 256MB $, which is much larger compared to the block size of the nested loop according to figure~\ref{fig-L3Prof} (b), so in this scenario, L3 capacity has minor influence on overall performance.
\begin{figure}[h]
    \centering
    \includegraphics[width=0.49\linewidth]{VersionShifting-eps-converted-to.pdf}
    \includegraphics[width=0.49\linewidth]{PS-IT-eps-converted-to.pdf}
    % OneDrive/MultiVersion/Strategy_plot/plot2.py
    % OneDrive/MultiVersion/auto_scheduler/extract_comp_flag.py
	\caption{\label{fig-MultiVersionFinding} (a) We observe the situation of version switching from no interference and heavy interference, most of operators switch to the version with larger blocking size and smaller parallel/unroll width, some of the operators have contrast trend, that's because the version used in this experiment are found with no heuristic info, the versions of these operators are much more homogeneous, thus making it no benefit using multi-version. \FIXME{Should abandon, (b) We measure the actual performance of found implementations and observe strong relation between interference tolerance and parallel scalability, which matches the compiling flags, add a figure showing the identical L3 bandwidth and Cache Miss of different core number.}}
\end{figure}
\begin{figure}[h]
    \centering
    \includegraphics[width=0.47\linewidth]{L3CATTrend.pdf}
    \includegraphics[width=0.52\linewidth]{L3Cap.pdf}
    % OneDrive/MultiVersion/Strategy_plot/plot2.py
    % OneDrive/MultiVersion/auto_scheduler/extract_comp_flag.py
	\caption{\label{fig-L3Prof} (a) We use Intel Cache Allocation Technology (CAT) to limit the L3 cache capacity (cache line) and evaluate the performance of operators, most of operators have almost no performance downgrade when decreasing L3 cache capacity. (b) We observe the data size per block of all implementations and find that they are lower than hardware L3 cache capacity by 3 to 7 magnitude.}
\end{figure}
Combining previous findings, to find candidate operators implementation, we use the blocking/tiling size and parallel/unroll width as our heuristic. Following several steps, we can get multiple versions for interference handling (The detailed algorithm are listed in algorithm~\ref{Algo-FindingVersion}):
\begin{itemize}
    \item Calculate the minimal float point performance $ min\_perf_{t} $ to satisfy the QoS target $ qos_{t} $ by $ min\_perf_{t}=\frac{\sum_{j\in\lbrack 1, t.length \rbrack}}{qos_{t}} $.
    \item Select all the samples that outperform the $ min\_perf_{t} $ from the log generated by the auto-scheduler.
    \item Mark all dominant samples $ s_{d} $ so that $ \nexists s\in\lbrace samples \rbrace, s.t.~s_{d}.Parallel<s.Parallel~\&\&~s_{d}.BlockingSize<s.BlockingSize $.
    \item Choose the sample from all dominant samples and compile them to implementations following a step (which is a meta-parameter of how many different implementations the system uses to handle different interference, the more the better, but increasing implementations loaded to the memory will increase memory footprint.)
\end{itemize}
To verify that finding implementation version by compiling flag have actual result in tolerating interference, we observe the performance counters measured when actually executing these implementations with interference, illustrated in figure~\ref{fig-MultiVersionFinding} (b). When we choose the implementation with larger blocking size, which imply it has lower parallel scalability, it out perform other implementations when facing heavy interference, which match the compiling flag well.

\PBox {
    \textbf{Core Insight B}: Scheduling tasks at sub-model grain can not only reduce response latency and conduct more efficiency resource allocation but also avoid frequent resource allocation conflict.
}
\subsubsection{Forming and Scheduling Sub-Model at Runtime}
After the candidate implementations are found, we should find out how to form the sub-model and how to allocate resources to them. According to our observations in finding implementation versions, implementations with different interference tolerance abilities have different parallel scalability, thus different CPU core number preferences. Since we want to smooth the fluctuating CPU core allocation, reduce the CPU core allocation conflict, we should allocate the same CPU core resource to operators in a sub-model. Which imply we should put operators with similar CPU core preference into a sub-model. So, we first profile the performance of implementations in various CPU core usage, and collect the core number requirement of different implementations of one operator as listed in table~\ref{tab-example}. We found that there exists strong spatial similarity in core number preference of operators in the deep learning model, as illustrated in figure~\ref{fig-FormingSubModel} (a).
% \begin{table}[h]
% 	\caption{\label{tab-example} CPU Core requirement of implementations of the first operator of task $ t $ ($ t=ResNet-50 $)}
% 	\begin{center}
% 	\begin{tabular}{|c|c|c|c|c|}
% 	    \hline
% 	    $ qos_{t}\lbrack 0 \rbrack $ & \tabincell{c}{Ver.\\ID} & \tabincell{c}{Block\\Size} & \tabincell{c}{Parallelizing} & \tabincell{c}{CPU Core\\Requirement}\\
%         \hline
%          & 1 & 1 & 1 & 16\\
%          & 2 & 1 & 1 & 24\\
%         0.289 ms & 3 & 1 & 1 & 16\\
%          & 4 & 1 & 1 & 32\\
%          & 5 & 1 & 1 & 24\\
%         \hline
%     \end{tabular}\\
%     \end{center}
% \end{table}
\subsubsection{Scheduling Strategy Algorithm List}
\begin{algorithm}[h]
	\caption{Finding candidate implementations of layers in a task template at compiling stage.}
	\label{Algo-FindingVersion}
	\textbf{Input:}  $ layers\lbrack 1:N \rbrack $, $ qos $\\
	\textbf{Output:}  $ candidate\_impl\lbrack V \rbrack $, $ dominant\_impl\lbrack  \rbrack $
	\begin{algorithmic}[1]
		\Function {FindingImpl}{$ layers\lbrack 1:N \rbrack $, $ qos $}
        \For {$ \_l $ \textbf{in} $ layers \lbrack 1:N \rbrack$}
        \State {$ \_l.qos\leftarrow qos\times \frac{\_l.op\_count}{\sum_{x\in layers\lbrack 1:N \rbrack}(x.op\_count)} $}
        \State {$ impls\lbrack  \rbrack\leftarrow Ansor(\_l, 1024) $}
        \State {$ impls\lbrack  \rbrack\leftarrow \lbrack x.time\leq \_l.qos~for~x~in~impls \rbrack $}
        \State {$ d\_impl\lbrack  \rbrack\leftarrow ExtractDominant(impls) $}
        \State {$ d\_impl\lbrack  \rbrack.sort(key=x.block\_size) $}
        \For {$ \_i $ \textbf{in} $ d\_impl, step\leftarrow\frac{d\_impl.length}{V} $}
        \State {$ candidate\_impl.push\_back(\_i) $}
        \EndFor
        \EndFor
        \State \Return {$ candidate\_impl\lbrack V \rbrack $, $ d\_impl\lbrack  \rbrack $}
		\EndFunction
		
		\Function {ExtractDominant}{$ impls\lbrack  \rbrack $}
		\State {$ d\_impl\leftarrow \lbrack  \rbrack $}
		\For{$ i $ \textbf{in} $ impls $}
		\State {$ isDominant\leftarrow True $}
		\For{$ j $ \textbf{in} $ impls $}
		\If {$ i==j $: \textbf{continue}}
		\EndIf
		\If {$ j.block\_size \geq i.block\_size $ \textbf{and} $ j.parallel \geq i.parallel $}
		\State {$ isDominant\leftarrow False $, \textbf{break}}
		\EndIf
		\EndFor
		\If{$ isDominant==True $}
		\State {$ d\_impl.push\_back(i) $}
		\EndIf
		\EndFor
		\State \Return {$ d\_impl $}
		\EndFunction
	\end{algorithmic}
\end{algorithm}




